Embeddings for Tabular Data: A Survey

Tabular data comprising rows (samples) with the same set of columns (attributes, is one of the most widely used data-type among various industries, including financial services, health care, research, retail, and logistics, to name a few. Tables are becoming the natural way of storing data among various industries and academia. The data stored in these tables serve as an essential source of information for making various decisions. As computational power and internet connectivity increase, the data stored by these companies grow exponentially, and not only do the databases become vast and challenging to maintain and operate, but the quantity of database tasks also increases. Thus a new line of research work has been started, which applies various learning techniques to support various database tasks for such large and complex tables. In this work, we split the quest of learning on tabular data into two phases: The Classical Learning Phase and The Modern Machine Learning Phase. The classical learning phase consists of the models such as SVMs, linear and logistic regression, and tree-based methods. These models are best suited for small-size tables. However, the number of tasks these models can address is limited to classification and regression. In contrast, the Modern Machine Learning Phase contains models that use deep learning for learning latent space representation of table entities. The objective of this survey is to scrutinize the varied approaches used by practitioners to learn representation for the structured data, and to compare their efficacy.

==> sections/coursework.tex <==
\noindent
\textbf{\huge{Course Work Details}}
\vspace{25 pt} \\
\textbf{\large{Name : Rajat Singh}}
\vspace{20 pt} \\
\textbf{\large{Entry Number : 2020CSZ8507}}
\vspace{20 pt} \\
\textbf{\large{Date of Joining : 28 September, 2020}}

\begin{center}
    \begin{tabular}{p{0.8cm} p{1.8cm} p{8.5cm} p{1.8cm} p{1cm} p{1cm}} 
    \hline \\ 
    \textbf{S.No.} & \textbf{Course ID} & \textbf{Course Name} & \textbf{ Bucket} & \textbf{Grade} & \textbf{Credits}\\ [1 ex] 
    \hline \\
    1 & COL702 & ADVANCED DATA STRUCTURES &  & C & 4.0 \\ 
    2 & COL764 & INFORMATION RETRIEVAL AND WEB SEARCH & Application & B & 4.0 \\
    3 & COL819 & ADVANCED DISTRIBUTED SYSTEM & System & A- & 4.0 \\
    4 & COL873 & SPECIAL TOPICS IN NATURAL LANGUAGE PROCESSING & Audit & NP & 3.0 \\ 
    5 & COL759 & CRYPTOGRAPHY AND COMPUTER SECURITY & Theory & A- & 3.0\\
    6 & HSL800 & RESEARCH WRITING & Audit & NP & 3.0 \\
    7 & COL761 & DATA MINING & & B & 4.0 \\
    8 & SIV895 & SPECIAL MODULE ON INTELLIGENT INFORMATION PROCESSING & & A- & 1.0 \\
    9 & COL865 & SPECIAL TOPICS IN COMPUTER AP. & & & 3.0\\
    \hline
    \end{tabular}
    \vspace{10 pt}
\end{center}
\textbf{\large{Credits Earned : 20}}
\vspace{20 pt} \\
\textbf{\large{CGPA : 8.0}}


==> sections/proposal.tex <==
\section{Proposed Work}
\label{sec:proposal}

This section we outline the possible future research directions, which addresses the limitations of the existing work.

\subsection{Problem Statement 1: Learning Embeddings on Multi-tabular Databases (\ourm)}

\subsubsection{Current Progress}
We (joint work with Garima Gaur, Vinayak Gupta, Siddhant Arora and Srikanta Bedathur) started the initial work on this problem and our paper got accepted  in CoDS-COMAD titled: “Teaching Old DB Neu(ral) Tricks: Learning Embeddings on Multi-tabular Databases”.

% \sbjnote{Expand this further - you have a lot of material in the paper that could be utilized here}
%\textbf{Problem Statement 1}: Learning Embeddings on Multi-tabular Databases (Relbert)\\

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=\columnwidth]{images/Intro.pdf}
%    \caption{Schematic diagram of embedding learning procedure of \ourm for two tables from the IMDB dataset.}
%    \label{fig:intro}
%\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.8\columnwidth]{images/relbert_main.pdf}
\caption{Schematic diagram of the embedding procedure in \ourm.}
\label{fig:MLM_Encoder}
\end{figure}

% \sbjnote{Do not make these as items -- if required you should make them subections. Better may be to simply make them paragraphs \rsjnote{done}}

% \sbjnote{I do not see any examples here -- what classification task and imputation task would be required here? Also, there were some comments by reviewers on the baselines from traditional data imputation frameworks. I am sure your examiners will ask the same question.}

% \sbjnote{You may also want to mention your MICCAI work here.}

    \subsubsection{Motivation}
    
    % There are several issues associated with tabular data (\hyperref[sec:challenges]{Section 2}), ranging from data quality to domain-specific terminology. In this work, we address some of these issues, including multiple semantics for the same token and domain-specific vocabulary, and propose a deep learning model that consider these issues and learns a better representation for tabular data. 
    
    The majority of valuable data is still stored in traditional relational databases. In particular, data-centric applications like e-commerce, finance, and organization management systems, are powered by enterprise database engines like IBM DB2, Apache Derby, Monet DB, Oracle DB, etc. However, the research question of employing ML models to improve the standard database issues like missing value imputation, data integration, classification, and so on, is under-explored. It can be explained by the scarcity of robust representation learning approaches for relational databases.
    
    Most of the approaches \cite{TabFact, TURL} either work with web-tables and, thus, do not deal with the intricacies of a relational database or, even if they work with the relational data, they fail to fully leverage the implicit knowledge a database schema captures about the stored data. In this work, we do not treat entities just as a simple word in a NL sentence rather, we focus on their semantics. For instance, if a syntactically same entity is present in two different columns, we treat them as two separate entities mapped to two different column aware latent spaces. 
    
    
    
    \subsubsection{Task} 
    The tasks on which we evaluate the quality of the embeddings generated by this model are classification and Missing Value Imputation (MVI). Classification - in this task, given a tuple of the table, we would like to assign a class to that tuple based on the contents of the tuple. Missing Value Imputation (MVI) - in this task a random cell value will be missing from the tuple of the table and model needs to predict the cell value corresponding to that missing cell in the tuple.
    
    
    \subsubsection{Datasets} 
    The datasets that we used for the above task including IMDb\footnote{https://relational.fit.cvut.cz/dataset/IMDb} Dataset and MIMIC \cite{mimic} Clinical Dataset. Where, MIMIC \cite{mimic} is a health-related relational database consisting of 26 tables. It consists of the health record of over 40,000 patients who stayed in critical care units of the Beth Israel Deaconess Medical Center between 2001 and 2012. In contrast, the IMDb dataset is a movies-related relational database consisting of 7 tables connected with each other using FK-PK join as shown in figure \ref{fig:imdb_schema}.  
    
    If we look closely, both datasets are completely different in terms of content. Both datasets have very domain-specific vocabulary; thus, we can't use pre-train models as those models might not contain the vocabulary present in these domain-specific datasets.
    
    \begin{figure}[htp]
        \centering
        \includegraphics[width=0.8\columnwidth]{images/imdb_schema.png}
        \caption{IMDb dataset schema.(https://relational.fit.cvut.cz/dataset/IMDb)}
        \label{fig:imdb_schema}
    \end{figure}
    
    \subsubsection{Model}
    
    For any table $\bs{T}$, our model incorporates a self-attention model for encoding the entities in a table. Rows of the table are used to generate sentences, which are then fed sequentially into the transformer. However, unlike a natural language sentences, each word in a table row belongs to a column in that table, and each column inherently contains distinct entity information. For instance, an entity in the actor column captures entirely different semantics as compared to the identical entity in the director column. Thus, a homogeneous embedding initialization function will fail to incorporate the column heterogeneity. 
    
    For this, we propose $\ourm$, to learn column-aware semantic representation for each entity in a relational table. We treated each tuple of the table as a sentence and fed these sentences to the transformer. We use distinct embedding space corresponding to each column in the table ($\bs{T}$) denoted by $\Phi$ (Figure \ref{fig:MLM_Encoder}). The embedding matrix for the entities in the table can be calculated as follows:
        
    \begin{equation}
        \bs{P}^k_i = \Phi^{k}(val_{k}^{i}), \qquad \forall val_{k}^{i} \in \bs{T},
    \end{equation}
    
    where $\Phi^k$ and $i$ denote embedding function for $k$-th column and the row (or sentence) index in the relational table, respectively. As in \cite{BERT}, we use \textit{Mask Language Model (MLM)} and \textit{Next Sentence Prediction (NSP)} as the learning objectives for the transformer. Thus, $\ourm$ parameters are optimized by minimizing the net loss, which is the sum of the respective MLM and NSP cross-entropy losses.
    
    \begin{equation}
        \cm{L}_{A} = \cm{L}_{mlm} + \cm{L}_{nsp},
    \end{equation}
    
    
    
    \subsubsection{Results} As shown in Table \ref{tab:mvi}, we tested our model for MVI over IMDb and MIMIC datasets against Table2Vec \cite{table2vec} and EmbDI \cite{embdi} and $\ourm$ outperform the Table2Vec and EmbDI. In addition, Table \ref{tab:class-imdb} and Table \ref{tab:class-mimic} show the results for classification task. In addition, table \ref{tab:e1} shows the performance of $\ourm$ and a model that finetunes the pretrained BERT, whereas \ref{tab:e2} compatre the performance of the $\ourm$ with the $\ssrel$ that embds all the tokens to a same latent space. The experimental results have reaffirmed the superiority of attention models for the embedding learning task and further verified our central concept of embedding distinct columns into distinct latent spaces.
    
    \begin{table} [t]
        \centering
        \begin{tabular}{@{}l| l l l| l l l @{}} 
        \toprule
        \multirow{2}{*}{Approach} & \multicolumn{3}{c}{IMDB} & \multicolumn{3}{c}{MIMIC}\\ \cline{2-7}
         & MR & MRR & Hit@10 & MR & MRR & Hit@10 \\
        \midrule
        \tabvec & ${44.252}$ & ${0.0631}$ & ${0.176}$ & ${657.022}$ & ${0.206}$ & ${0.663}$ \\ 
        \embdi & ${52.302}$ & ${0.036}$ & ${0.0792}$ & ${1036.53}$ & ${0.175}$ & ${0.6197}$  \\
        \ourm & $24.976$ & $0.16$ & $0.321$ & $205.576$ & $0.64$ & $0.906$\\
        \bottomrule
        \end{tabular}
        \caption{MVI task performance comparison of {\ourm} against other baselines over {\imdb} and \mimic.}
        \label{tab:mvi}
    \end{table}
    
    
    \begin{table} [t]
        \centering
        \begin{tabular}{@{}l| c c | cc| cc |cc @{}} 
         \toprule
         
         \multirow{2}{*}{Approach} & \multicolumn{2}{c}{k=5} & \multicolumn{2}{c}{k=10} & \multicolumn{2}{c}{k=15} & \multicolumn{2}{c}{k=20} \\ \cline{2-9}
          & $P$ & $R$ & $P$ & $R$ & $P$ & $R$ & $P$ & $R$ \\ 
          \midrule
         
         \tabvec & ${0.07}$ & ${0.20}$ & ${0.07}$ & ${0.40}$ & ${0.08}$ & ${0.64}$ & ${0.09}$ & ${1}$ \\ 
         \embdi & $0.03$ & $0.07$ & $0.04$ & $0.24$ & $0.06$ & $0.47$ & $0.09$ & $1$ \\
         \ourm  & $0.048$ & $0.08$ & $0.065$ & $0.24$ & $0.09$ & $0.56$ & $0.11$ & $1$ \\
         %\multirow{2}{*}{Approach} & \multicolumn{3}{c}{\imdb} & \multicolumn{3}{c}{\mimic}\\ \cline{2-7}
         \bottomrule
        \end{tabular}
        \caption{Classification task performance comparison (micro precision $P@k$ and recall $R@k$)of \ourm against other baselines over IMDb.}
        \label{tab:class-imdb}
    \end{table}
 

     \begin{table} [htp]
        \centering
        %\resizebox{\columnwidth}{!}{  
        \begin{tabular}{@{}l| c c | cc| cc @{}} 
         \toprule
          \multirow{2}{*}{Approach} & \multicolumn{2}{c}{k=1} & \multicolumn{2}{c}{k=3} & \multicolumn{2}{c}{k=5} \\ \cline{2-7}
          & $P$ & $R$ & $P$ & $R$ & $P$ & $R$  \\ 
          \midrule
         \tabvec & ${0.22}$ & ${0.22}$ & ${0.21}$ & ${0.64}$ & ${0.20}$ & ${1}$ \\ 
         \embdi & ${0.44}$ & ${0.44}$ & ${0.28}$ & ${0.84}$ & ${0.20}$ & ${1}$  \\
         \ourm  & $0.58$ & $0.58$ & $0.32$ & $0.97$ & $0.2$ & $1$  \\
         \bottomrule
        \end{tabular}%}
        \caption{Classification task performance comparison (micro precision $P@k$ and recall $R@k$) of \ourm against other baselines over \mimic.}
        \label{tab:class-mimic}
    \end{table}
    
     \begin{table} [htp]
        \centering
        \begin{tabular}{@{}l| l l l| l l l @{}} 
         \toprule
         \multirow{2}{*}{Approach} & \multicolumn{3}{c}{\imdb} & \multicolumn{3}{c}{\mimic}\\ \cline{2-7}
         & MR & MRR & Hit@10 & MR & MRR & Hit@10 \\
         \midrule
         Finetuned BERT & $1182.308$ & $0.086$ & $0.207$ & $1105.55$ & $0.07$ & $-$ \\ 
        \ourm & $24.976$ & $0.16$ & $0.321$ & $205.576$ & $0.64$ & $0.906$\\\bottomrule
        \end{tabular}
        
        \caption{Performance comparison of {\ourm} and a model that finetunes the pretrained BERT with natural language sentences constructed using the tabular data.}
        \label{tab:e1}
    \end{table}
    
    
     \begin{table} [htp]
        \centering
        \begin{tabular}{@{}l| l l l| l l l @{}} 
         \toprule
         \multirow{2}{*}{Approach} & \multicolumn{3}{c}{\imdb} & \multicolumn{3}{c}{\mimic}\\ \cline{2-7}
         & MR & MRR & Hit@10 & MR & MRR & Hit@10 \\
         \midrule
         \ssrel & $56.46$ & $0.069$ & $0.154$ & $500.802$ & $0.229$ & $0.544$ \\ 
         \ourm & $24.976$ & $0.16$ & $0.321$ & $205.576$ & $0.64$ & $0.906$\\
        \bottomrule
        \end{tabular}
        \caption{Performance comparison of $\ourm$ and $\ssrel$ that embeds all the tokens to a same latent space.}
        \label{tab:e2}
    \end{table}

    
    \subsubsection{Future Work} In this work, we revolve around classification and missing value imputation (MVI) task. Further, we want to explore how this column-aware semantic representation performs for more complex tasks such as Table Question Answering. Another line of work that is in continuation of the above problem setting is MICCAI\footnote{https://2022.miccai-hackathon.com/} 2022 hackthon task 3, where the task was to classify the risk of the patient based on the medical report readings of that patient. The dataset have three kind of reports (blood values, radiology and temperature) for each patient and a target risk level based on the reports. Each report is a tabular data with an additional semantic i.e., timestamp of the test as shown in figure \ref{fig:miccai_dataset_rp1} \ref{fig:miccai_dataset_rp2} \ref{fig:miccai_dataset_rp3}.  These tables also contain missing values. We can also extract similar kind of dataset from MIMIC-IV\footnote{https://physionet.org/content/mimiciv/0.4/} dataset.
    
    \begin{figure}[htp]
        \centering
        \includegraphics[width=1.0\columnwidth]{images/miccai_dataset_1.png}
        \caption{MICCAI dataset: Blood report of a patient}
        \label{fig:miccai_dataset_rp1}
    \end{figure}
    
    
     \begin{figure}[htp]
        \centering
        \includegraphics[width=1.0\columnwidth]{images/miccai_dataset_2.png}
        \caption{MICCAI dataset: Radiology report of a patient}
        \label{fig:miccai_dataset_rp2}
    \end{figure}
    
     \begin{figure}[htp]
        \centering
        \includegraphics[width=1.0\columnwidth]{images/miccai_dataset_3.png}
        \caption{MICCAI dataset: Temperature report of a patient}
        \label{fig:miccai_dataset_rp3}
    \end{figure}
    
    
% \subsubsection{Contribution}

%\subsubsection{Table Encoder}
%For any table $\bs{T}_{\bullet}$, our model incorporates a self-attention model for encoding the entities in a table. Rows of the table are used to generate sentences, which are then fed sequentially into the transformer. However, unlike a natural language sentences, each word in a table row belongs to a column in that table, and each column inherently contains distinct entity information \textcolor{red}{and its own vocabulary}. In Figure\ref{fig:intro}, for instance, an entity in the \textit{actor} column captures entirely different semantics as compared to the identical entity in the \textit{director} column. Thus, a homogeneous embedding initialization function will fail to incorporate the column heterogeneity. Therefore, we use distinct embedding spaces corresponding to each column in the table denoted by $\Phi^{\bullet}$ (Figure \ref{fig:MLM_Encoder}). We calculate the embedding matrix for the entities in the table as:

%\begin{equation}
%\bs{P}^k_i = \Phi^{k}(val_{k}^{i}), \qquad \forall val_{k}^{i} \in \bs{T},
%\end{equation}

%where $\Phi^k$ and $i$ denote embedding function for $k$-th column and the row (or sentence) index in the relational table respectively. Following \cite{BERT}, we utilize a masked-language based learning where we randomly mask one of the entities in a sentence and then predict those masked entities based on the transformer output. We compute the output embeddings for each entity through an encoder network consisting of multiple attention layers. We denote the output embeddings for each sentence indexed by $i$ as $\bs{O}_i = \texttt{TEncoder} (\bs{P}_i)$, where $\texttt{TEncoder}(\bullet)$ denotes the base-transformer module. However, since each column $k$ has a different embedding space, computed by $\Phi^k$, we determine the candidate entities for the \textit{masked} entity in the sentence using an output-softmax over the entities in the column of the masked entity. We learn the parameters for the horizontal transformer by optimizing the cross entropy loss function for each sentence in the table $\bs{T}$ as:

%\begin{equation}
%\cm{L}_{mlm} = \sum_{i=1}^{|\bs{T}|}\texttt{CrossEntropy}(\bs{o}^{m}_i, %\bs{P}^{mask}_i), \qquad \bs{o}^m_i \in \bs{O},
%\end{equation}

%where, $\bs{o}^m_i, \bs{P}^{mask}$ denote the output embedding corresponding to the masked index and the column entities respectively. In addition, we exclude positional embeddings from the transformer model as a table is inherently \textit{permutation-invariant}. We initialize each entity in a row of the table using standard word2vec \cite{Word2vec} computed over the table by simply treating each row as a sentence.

%\subsubsection{\ourm}

%$\ourm$ learns column-aware, semantic representations for each entity in a relational table. However, a relational table is organized into multiple tables, either to efficiently enforce integrity constraints or to enhance the overall database efficiency using the \emph{data normalization} process. Therefore, in order for \ourm to learn semantic information between two linked entities spread across the tables, it requires information from multiple tables. For instance, actor-genre in actor tables and director-genre in director table contribute to modelling the genre-preference for both entities, which could assist a director in finding a plausible actor for his/her movie.

%However, learning entity representations across multiple tables incurs a high computational cost due to the need to compute (explicitly or implicitly) all pairs of fk-pk joins between tables, commonly known as \textit{denormalization} of the database. Secondly, a denormalized table degrades the data quality since it may merge unrelated attributes and dramatically increase table size by repeating the rows of the table multiple times. 

%To circumvent these bottlenecks, we model the table joins as a \textit{next-sentence prediction} problem. Specifically, consider two tables $\bs{T}_{\alpha}$ and $\bs{T}_{\beta}$ that can be joined via the primary-key column $\bs{c}_A^{\alpha}$ in table $\bs{T}_\alpha$, and the corresponding \textit{foreign-key} column $\bs{c}_{\hat{A}}^\beta$ in table $\bs{T}_\beta$. If a row containing entity $val_{c_\alpha}^i \in \bs{c}_A^\alpha$ is linked to the row containing entity $val_{c_\beta}^j \in \bs{c}_{\hat{A}}^\beta$, then the latter is considered as the \textit{next sentence} for the current row. In addition, we generated sentence pairs from these rows by separating them with [SEP] token and appending [CLS] and [SEP] tokens in the beginning and end, respectively. This sentence pair is later fed into \ourm to learn inter-table information for an entity. We utilize the output embedding at the $\texttt{[CLS]}$ token to estimate the probability of a sentence being the \textit{next} sentence, $v_{t_i^\alpha, t_j^\beta}$  and use a negatively sampled row $t'^\beta_j \in \bs{T}_\beta$. The loss for NSP is calculated via:

%\begin{equation}
%\cm{L}_{nsp} = -\sum_{i=1}^{|\bs{T}_\alpha|} \sum_{t_i^\alpha \in \bs{T}_\alpha} \left[ \log \left ( \sigma(v_{t_i^\alpha, t_j^\beta}) \right) + \log \left (1 - \sigma(v_{t_i^\alpha, t_j^{'\beta}}) \right) \right],
%\end{equation}

%where $t_i^\alpha$ and $t_j^\beta$ are $i^{th}$ and $j^{th}$ row in $\bs{T}_\alpha$ and $\bs{T}_\beta$ tables respectively and $\sigma$ denote the \textit{sigmoid} function. Finally, we combine this next sentence prediction task with the mask language model learning of the predefined table encoder.

%\subsubsection{Optimization}

%Training {\ourm}  for table MLM enables us to learn relationships between attributes whereas the NSP task helps to aggregate inter table information i.e. join between the tables. By introducing the next sentence prediction task, we develop the first table auto-completion approach that avoids the bottlenecks of a denormalised table. 
%{\ourm} parameters are optimised by minimising the net loss, which is the sum of the respective MLM and NSP cross entropy losses.
%\begin{equation}
%\cm{L}_{A} = \cm{L}_{mlm} + \cm{L}_{nsp},
%\end{equation}
%However, joining different tables at each training iteration would lead to an information loss over multiple iterations. Therefore, our training strategy consists of a two-step approach, with the first step as general \textit{pre-training} step which is followed by task-specific \textit{fine-tuning}.\\

%\noindent
%\textit{Pre-training:} To understand the relationships between tables and attributes during pre-training, we perform a task-independent learning of all entities in the database. Specifically, we construct pairwise sentences between tables using the primary-key joins in the relational schema and train the model parameters using standard MLM-based optimization.\\

%\noindent
%\textit{Fine-Tuning:} The pre-training step is followed by task-specific \textit{fine-tuning} of the model. More so, for our task of table auto-completion we jointly fine-tune the {\ourm} model to predict the \textit{masked} entity for each row and simultaneously the join-based next sentence by optimizing the net loss $\cm{L}_{A}$.


%\noindent
% We evaluated the quality of the embeddings generated via the task of missing value imputation via cell value prediction, i.e. model predicts the token corresponding to an empty cell. We report the performance of baseline systems and our proposed framework {\ourm} in Table \ref{tab:mvi}. 
%Note that for {\mimic} dataset, while the mean rank (MR) of {\embdi} is poor as compared to that of $\tabvec$, their $Hit@10$ percent is comparable. This point towards the disparity in the prediction capability of $\embdi$. While it is performing better in certain cases, it is ranking the other ones badly. In contrast, $\ourm$, has a consistent performance as its MR is lowest in comparison of all other systems and for almost one third of the predictions, the answers are listed correctly in top-10 predicted tokens. $\ourm$ showcased an reduction of about $52\%$ and $79\%$ in the mean rank from that of $\embdi$ over $\imdb$ and $\mimic$ datasets respectively. 

% Interestingly, the performance of $\ourm$ over $\imdb$ and $\mimic$ datasets is not comparable, i.e. $\ourm$ is not clearly performing better on one dataset than the other. While the \emph{mean rank} for $\imdb$ is quite low as compared to that for $\mimic$, the $Hits@10$ for $\mimic$ is significantly high in comparison to $\imdb$. This pattern indicates that $\ourm$ favours some columns over the other. The low MR  for $\imdb$ indicates the column (tokens) in $\imdb$ are equally easy to predict, whereas $\mimic$ columns are either very easy or too tough to predict correctly. This can explain the undesirable high MR and  desirable high $Hit@10$ on the $\mimic$ database. 


\subsection{Problem Statement 2: Complex Question Answering over table}


    \subsubsection{Motivation} Question answering is one of the most intuitive tasks for humans but a complex task for machines. TAPAS \cite{tapas}, and TaBert \cite{tabert} are some early works in the field of table question answering. TaBert uses content snapshots based on n-gram matching to select the initial tuples that are relevant for the final answer. N-gram matching has a very high chance of failure for complex question answering. Whereas, TAPAS \cite{tapas} works with QA over single tables, there are two type of questions present in TAPAS one is aggregation question and other are simple questions as shown in figure \ref{fig:wrestling}. TAPAS can deal with three kind of aggregation questions i.e., SUM, AVG and COUNT. But the real world tables can have more complex question such as "Number of employees with the salary greater than the salary of Aman?" or "Which product is having the same seller as 'product-xyz?'". In this scenario we are not asking a direct question but an indirect question. Thus we would like to explore a better approach for these type of complex question answering over the tabular data.
    
    \subsubsection{Task} Question Answering: Given a set of relational tables and a natural language (NL) Question, we would like to get the answer to the given NL query based on the given set of tables.
    
    \begin{figure}[htp]
        \centering
        \includegraphics[width=0.6\columnwidth]{images/hybridQA.png}
        \caption{The type of questions in HybridQA \cite{hybrid_qa}}
        \label{fig:hybridQA}
    \end{figure}
    
    \subsubsection{Datasets} WikiTables \cite{wikitables} and HybridQA \cite{hybrid_qa} for testing our model. WikiTables contain 1.6M tables with surrounding text about the Wikipedia page it has been extracted, such as caption, page title, and section title. It also comes with table metadata such as the number of columns, column datatypes, rows, etc. Whereas, HybridQA is a smaller dataset as compared to WikiTables. It contains 13K tables with questions and some text related to the table. Figure \ref{fig:hybridQA} shows the type of questions in the HybridQA dataset.
    
   % \sbjnote{This is not the way to present the datasets. You also need to give the reference to the paper which introduced this dataset. \rsjnote{done}}
    

\subsection{Problem Statement 3: Hybrid models for multi-tabular data}

%\begin{figure}[htp]
%    \centering
%    \includegraphics[width=0.6\columnwidth]{images/task2_1.png}
%    \caption{Snapshot of a table}
%    \label{fig:task2_1}
%\end{figure}



\begin{figure}[htp]
    \centering
    \includegraphics[width=0.9\columnwidth]{images/multi-tables.png}
    \caption{Multi-tabular schema}
    \label{fig:task2_1}
\end{figure}

    \subsubsection{Motivation} 
    
    %Real-world tables are heterogeneous in nature, i.e., the features are of different scales, types, and meaning. For example, as shown in Figure \ref{fig:task2_1}, the cell with entity 78 in \textit{Age} column is entirely different in semantics from the cell with entity 78 in \textit{Weight} column. 
    In \cite{boost_then_convolve}, authors introduce the hybrid models and shows that decision trees alone work well with small and heterogeneous tabular data, whereas deep-learning models alone work well with large and homogeneous tabular data. But they can combine the benefits of both using hybrid models. Authors in \cite{boost_then_convolve} uses only single table for their task of classification and regression but real world databases are multi-tabular in nature i.e, data is distributed into multiple tables and the tuples in these tables are connected using joins (figure \ref{fig:task2_1}) and also heterogeneous in nature. Thus, in this work, we would like to explore more about hybrid models (a combination of classical models and deep learning models ) for learning better representations of heterogeneous multi-tabular data for various downstream tasks.
    
    \subsubsection{Task} 
    Entity Linking: Let there are $T_1, T_2, ...., T_n$ tables and a new tuple comes in table $T_k$ then we want to predict the tuples in other tables that can be semantically linked with the given tuple in table $T_k$.\\
    Classification: Given the multi-tabular dataset we want to perform classification such that while training the model we need not to explicitly perform join over all the tables, as joining the tables can increase the redundancy and explode the size of the dataset.
    
    \subsubsection{Datasets} IMDb \footnote{https://relational.fit.cvut.cz/dataset/IMDb}, and MIMIC \cite{mimic} dataset
    
    \item \textbf{Open Problems}: 
    \begin{itemize}
        \item How to incorporate the heterogeneous tables with the deep learning model using tree-based models?
        \item How to train the hybrid model end-to-end?
        \item To what extent is the model scalable?
    \end{itemize}
     


%\subsection{Problem Statement 3: Data Integration: With ML perspective}

%\begin{itemize}

%    \item \textbf{Motivation}: 
    
%    \item \textbf{Task}:
    
%    \item \textbf{Datasets}: 
     
%\end{itemize}



% \subsection{Problem Statement 3: Rotation invariant for tabular data (using embdi + relbert)}




% \section{Current Progress}
% We started working on our first problem and have submitted a paper to CODS-COMAD 2022 titled: “Teaching Old DB Neu(ral) Tricks: Learning Embeddings on Multi-tabular Databases".

% \sbjnote{In many of the references below, you have no details of where they were published (e.g, URLNet, [23], [32], SAINT), Author names are messed up - sometimes in small letters, sometimes full list and sometimes not. Please clean up. \rsjnote{resolved}} 

% \sbjnote{How can [54] a master's thesis be coauthored by multiple people!!? \rsjnote{resolved}}

==> titlePage.tex <==
%% Define your thesis title, your name, your school, and your month and year of graduation here

% \newcommand{\thesisTitle}{Embeddings for \sout{Structured}Tabular Data}
\newcommand{\thesisTitle}{Embeddings for Tabular Data}
\newcommand{\yourName}{Rajat Singh}
\newcommand{\yourSchool}{Department of Computer Science and Engineering}
\newcommand{\yourclg}{Indian Institute of Technology Delhi}
\newcommand{\yourMonth}{November}
\newcommand{\yourYear}{2022}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Do not edit these lines unless you wish to customize
% the template
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{titlepage}
\begin{center}
\begin{singlespacing}

\LARGE\textbf{Survey}\\
\vspace{1\baselineskip}
\large \textbf{\textit{on}}\\
\vspace{1\baselineskip}
\LARGE\textbf{{\thesisTitle}}\\
\normalsize
\vspace{2\baselineskip}
\large \textbf{\textit{Submitted by}}\\
\vspace{1\baselineskip}
\LARGE\textbf{\yourName}\\
\large \textbf{2020CSZ8507}\\
\vspace{2\baselineskip}
\large\textbf{\textit{under the supervision of}}\\
\vspace{1\baselineskip}
\LARGE \textbf{Prof. Srikanta Bedathur}\\ 
\vspace{1\baselineskip}
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.28]{logo}
    
\end{figure}
\large
\textbf{\yourSchool}\\
\textbf{\MakeUppercase{\yourclg}}\\
%\vspace{\baselineskip}

\vspace{1\baselineskip}
\textbf{\yourMonth, \yourYear}

\end{singlespacing}

\end{center}
\texttt{}\end{titlepage}



